Speech-Copilot: Leveraging Large Language Models for Speech Processing via Task Decomposition, Modularization, and Program Generation

In this work, we introduce Speech-Copilot, a modular framework for instruction-oriented speech-processing tasks that minimizes human effort in toolset construction. Unlike end-to-end methods using large audio-language models, Speech-Copilot builds speech processing-specific toolsets by analyzing pre-collected task instructions and breaking tasks into manageable sub-tasks. It features a flexible agent based on large language models that performs tasks through program generation. Our approach achieves state-of-the-art performance on the Dynamic-SUPERB benchmark, demonstrating its effectiveness across diverse speech-processing tasks. Key contributions include: 1) developing an innovative framework for speech processing-specific toolset construction, 2) establishing a high-performing agent based on large language models, and 3) offering a new perspective on addressing challenging instruction-oriented speech-processing tasks. Without additional training processes required by end-to-end approaches, our method provides a flexible and extendable solution for a wide range of speech-processing applications.

==> images/image.tex <==
\begin{figure}[ht]
    \centering
    \includesvg[width=0.50\textwidth]{images/images/radar_reformat_v2.svg}
    \caption{Performance comparison of multiple models and our proposed pipeline across six aspects of Dynamic-SUPERB benchmark.}
    \label{fig:performance}
\end{figure}

==> tables/ablation_results.tex <==
\begin{table*}[th]
  \caption{Peformances of Speech-Copilot and the variant using multi-candidate program generation strategy on Dynamic-SUPERB.}
  \label{tab:dynamic-superb-ablation-result}
  \footnotesize
  \setlength{\tabcolsep}{5.3pt}
  \centering
  \begin{tabular}{ l | c  c  c  c  c  c | c}
    \toprule
    \multirow{2}{*}{\textbf{Model}} \\
     & {\textbf{Audio}} 
     & \textbf{Content} 
     & \textbf{Degradation}
     & \textbf{Paralinguistics} 
     & \textbf{Semantic} 
     & \textbf{Speaker} 
     & \textbf{Average} \\
    \# Tasks & 7 & 11 & 19 & 7 & 6 & 5 & 55 \\
    \midrule

    Original
    & 73.4
    & \textbf{90.7}
    & \textbf{64.3}
    & \textbf{56.6}
    & \textbf{70.7}
    & \textbf{86.1} 
    & \textbf{72.4} \\

    Multi-candidate
    & \textbf{75.5}
    & 87.6
    & \textbf{64.3}
    & 56.1
    & 68.5
    & \textbf{86.1}
    & 69.5 \\
    
    \bottomrule
  \end{tabular}
\end{table*}

% \cellcolor{orange!50}

==> tables/multicandidate.tex <==
\begin{table}[th]
  \caption{Peformances of Speech-Copilot and the variant using multi-candidate program generation strategy on Dynamic-SUPERB.}
  \label{tab:multi-candidate}
  \footnotesize
  \setlength{\tabcolsep}{5.3pt}
  \centering
  \begin{tabular}{ l | c  c}
    \toprule
    Aspects & Original & Multi-candidate \\
    \midrule
    \midrule
    Audio & 73.4 & \textbf{75.5} \\
    \midrule
    Content & \textbf{90.7} & 87.6 \\
    \midrule
    Degradation & \textbf{64.3} & \textbf{64.3} \\
    \midrule
    Paralinguistics & \textbf{56.6} & 56.1 \\
    \midrule
    Semantic & \textbf{70.7} & 68.5 \\
    \midrule
    Speaker & \textbf{86.1} & \textbf{86.1} \\
    \midrule
    \midrule
    Average & \textbf{72.4} & 69.5 \\
    
    \bottomrule
  \end{tabular}
\end{table}

% \cellcolor{orange!50}

==> tables/qwen_example.tex <==
\begin{table}[ht]
    \centering
    \caption{Example of the hallucination of Qwen-Audio-Chat.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c}
        \toprule
        \makecell[c]{Spoken content\\(Whisper output)} & \makecell[c]{Audio caption generated\\by Qwen-Audio-Chat} & \makecell[c]{Directly answer \\the question} \\
        \hline
        \hline
        \makecell[c]{hold said david \\ perceiving that \\...} & 
        
        \makecell[c]{The audio is of a man \\speaking, in a English, \\saying, \textbf{\color{teal}{``hold said david}} \\ \textbf{\color{teal}{perceiving that ..."}}.} & 
        
        \makecell[c]{The given text is ``such \\consumption as falls ..."\\ and the speech is \textbf{\color{red}{``such}} \\
        \textbf{{\color{red}{consumption as falls ..."}}}.\\ Therefore, the speech \\and text are congruent.}\\
        \bottomrule
    \end{tabular}
    }
    %\end{adjustbox}
    \label{tab:qwen_example}
\end{table}

==> tables/real_example.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \begin{tabular}{p{46em}}
    \toprule
    \textbf{User Instruction}  \\
    \midrule
    \texttt{Could you take a look at a voice message we received? We'd like to know what the person said, if it sounds like the usual person who calls us, and any interesting sounds in the background. Also, how did the caller seem to be feeling? It would be great if you could give us a full picture of the message.
    } \\ \\
    \midrule
    \textbf{Program Generation} \\
    \midrule
\begin{verbatim}
def main(audio_path, usual_caller_audio_path):
    # Transcribe the spoken words in the audio file to text
    transcription = speech_recognition(audio_path)

    # Verify if the voice in the message matches the usual caller
    same_person = speaker_verification(audio_path, usual_caller_audio_path)

    # Identify any interesting sounds in the background
    background_sounds = sound_classification(audio_path, "Identify any interesting sounds in the background.")

    # Recognize the emotions expressed by the caller
    emotion = emotion_recognition(audio_path)

    # Query LLM to get a full picture of the message
    query = f"The transcription of the message is: '{transcription}'. The caller is {'the usual person' 
        if same_person else 'not the 
        usual person'}. The background 
        sounds are: '{background_sounds}'. 
        The caller seems to be feeling: 
        '{emotion}'. Please provide a 
        full picture of the message."
    answer = query_llm(query)

    return answer
\end{verbatim} \\
    \midrule
    \textbf{Results} \\
    \midrule
    \texttt{Results here} \\
    \bottomrule
    \end{tabular}
    \caption{Real example}
    \label{tab:real example}
\end{table*}

